Type-directed Bounding of Collections in Reactive Programs

Our aim is to statically verify that in a given reactive program, the length of collection variables does not grow beyond a given bound. We propose a scalable type-based technique that checks that each collection variable has a given refinement type that specifies constraints about its length. A novel feature of our refinement types is that the refinements can refer to AST counters that track how many times an AST node has been executed. This feature enables type refinements to track limited flow-sensitive information. We generate verification conditions that ensure that the AST counters are used consistently, and that the types imply the given bound. The verification conditions are discharged by an off-the-shelf SMT solver. Experimental results demonstrate that our technique is scalable, and effective at verifying reactive programs with respect to requirements on length of collections.

==> base-type-checking-rules.tex <==
\begin{figure}[t]
	\scriptsize
	\centering
	\begin{mathpar}
		\inferrule* [Lab={\scriptsize BaseT-Add}]
		{
			\tycheck
			{\tyenv}
			{y: \trefine{\tlist{\basety}}{\kwrefine_y}}
			\\\\
			\tycheck
			{\tyenv}
			{x: \trefine{\basety}{\kwrefine_x}}
		}
		{
			\tycheck
			{\tyenv}
			{\eadd{y}{x}}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-Remove}]
		{
			\tycheck
			{\tyenv}
			{y: \trefine{\tlist{\basety}}{\kwrefine_y}}
		}
		{
			\tycheck
			{\tyenv}
			{\eremove{y}}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-Iter}]
		{
			\tycheck
			{\tyenv}
			{y: \trefine{\tlist{\basety}}{\kwrefine_y}}
			\\\\
			\tycheck
			{\tyenv}
			{z: \trefine{\titerator{\basety}}{\kwrefine_z}}
		}
		{
			\tycheck
			{\tyenv}
			{z = \eiterator{y}}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-AssignArith}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwint}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e_1: \trefine{\kwint}{\kwrefine_{e_1}}}
			\\
			\tycheck
			{\tyenv}
			{e_2: \trefine{\kwint}{\kwrefine_{e_2}}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e_1 \oparith e_2}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-AssignComp}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwbool}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e_1: \trefine{\kwint}{\kwrefine_{e_1}}}
			\\
			\tycheck
			{\tyenv}
			{e_2: \trefine{\kwint}{\kwrefine_{e_2}}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e_1 \opcomp e_2}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-AssignOr}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwbool}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e_1: \trefine{\kwbool}{\kwrefine_{e_1}}}
			\\
			\tycheck
			{\tyenv}
			{e_2: \trefine{\kwbool}{\kwrefine_{e_2}}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e_1 \lor e_2}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-AssignNeg}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwbool}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e: \trefine{\kwbool}{\kwrefine_e}}
		}
		{
			\tycheck
			{\tyenv}
			{x = \neg e}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-AssignInt}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwint}{\kwrefine_x}}
		}
		{
			\tycheck
			{\tyenv}
			{x = n}
		}
		\inferrule* [Lab={\scriptsize BaseT-AssignBool}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwbool}{\kwrefine_x}}
		}
		{
			\tycheck
			{\tyenv}
			{x = b}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-AssignIntX}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwint}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e: \trefine{\kwint}{\kwrefine_e}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-AssignBoolX}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\kwbool}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e: \trefine{\kwbool}{\kwrefine_e}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-AssignIter}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\titerator{\basety}}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e: \trefine{\titerator{\basety}}{\kwrefine_e}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-AssignList}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\tlist{\basety}}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{e: \trefine{\tlist{\basety}}{\kwrefine_e}}
		}
		{
			\tycheck
			{\tyenv}
			{x = e}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-Next}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\basety}{\kwrefine_x}}
			\\\\
			\tycheck
			{\tyenv}
			{z: \trefine{\titerator{\basety}}{\kwrefine_z}}
		}
		{
			\tycheck
			{\tyenv}
			{x = \enext{z}}
		}
				\\
		\inferrule* [Lab={\scriptsize BaseT-Decl}]
		{
			\forall \subastnode{\edecl{\ty}{x} = e}{P}.
			\tycheck{\tyenv}{x = e}
			\\\\
			\tycheck{\tyenv}{\stmt}
		}
		{
			\tycheck
			{\tyenv}
			{
				\overline{\edecl{\ty}{u}}\;
				\overline{\edecl{\ty}{x} = e}\;
				\stmt
			}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-NewList}]
		{
			\tycheck
			{\tyenv}
			{x: \trefine{\tlist{\basety}}{\kwrefine_x}}
		}
		{
			\tycheck
			{\tyenv}
			{x = \enewlist{\basety}}
		}
		\\
		\inferrule* [Lab={\scriptsize BaseT-Block}]
		{
			\overline{\stmt} = \stmt_1\cdots\stmt_n
			\\\\
			{\tycheck{\tyenv}{\stmt_i}}^{i \in 1\cdots n}
		}
		{
			\tycheck{\tyenv}{\eblock{s}}
		}\\
		\inferrule* [Lab={\scriptsize BaseT-While}]
		{
			\tycheck{\tyenv}{\stmt}
		}
		{
			\tycheck{\tyenv}{\ewhile{\expr}{\stmt}}
		}
		\inferrule* [Lab={\scriptsize BaseT-If}]
		{
			\tycheck{\tyenv}{\stmt_1}
			\\
			\tycheck{\tyenv}{\stmt_2}
		}
		{
			\tycheck{\tyenv}{\eif{\expr}{\stmt_1}{\stmt_2}}
		}
		\inferrule* [Lab={\scriptsize BaseT-Skip}]
		{
			{}
		}
		{
			\tycheck{\tyenv}{\eskip}
		}
	\end{mathpar}
	\caption{Base type checking rules}
	\label{fig:basetype-checking-rules}
\end{figure}


==> comments.tex <==
\small
%\begin{figure}[H]
%	\begin{tabular}{ l L L L}
%		Memory consumption & \memconsumestate{\env}{\cont}{\store}{state} & \bnfdef &
%		\sum_{x \in \domof{\env}}^{} \reachheap{x:\ty}{\env}{\store} + \memconsumestate{\env'}{\cont'}{\store}{},
%		\\
%		& & &
%		\hfill \text{where\;} \cont=\stackpush{\cont'}{\env'}
%		\\
%%		Live stack variables & \livevar{\env} & \bnfdef &
%%		\domof{\env}
%%		\\
%		Reachable heap size & \reachheap{x:\ty}{\env}{\store} & \bnfdef &
%		4
%		\text{,\;where\;} \ty=\kwint
%		\\
%		& & &
%		1
%		\text{,\;where\;} \ty=\kwbool
%		\\
%		& & &
%		\reachheap{v_1:\ty'}{\env}{\store}+\reachheap{v_2:\kwlist}{\env}{\store},
%		\\
%		& & &
%		\hfill \text{\;where\;} \ty=\kwlist \land \env[x]=\addr \land \store[\addr]=\scons{v_1}{v_2}
%		\\
%		& & &
%		\sum_{f \in C}^{} \reachheap{x.f:\ty_f}{\env}{\store}
%		\text{,\;where\;} \ty=C
%	\end{tabular}
%	\caption{Memory consumption of a concrete program state}
%	\label{fig:state-memory-consumption}
%\end{figure}
%
%
%\begin{figure}[H]
%	\begin{tabular}{ l L L L}
%		Peak memory consumption & \pmemconsume{P}{I} & \bnfdef &
%		\max(\memconsumestate{\env_1}{\cont_1}{\store_1}{state_1},
%		\memconsumestate{\env_2}{\cont_2}{\store_2}{state_2}, \cdots)
%		\\
%		& & &
%		\hfill \text{where $P$ stands for a program, $I$ stands for a}
%		\\
%		& & &
%		\hfill \text{particular input, and the execution trace is}
%		\\
%		& & &
%		\hfill (\emp, \emp, \emp) \xrightarrow[]{\stmt_1} (\env_1, \cont_1, \store_1) \xrightarrow[]{\stmt_2} (\env_2, \cont_2, \store_2) \xrightarrow[]{} \cdots
%	\end{tabular}
%	\caption{Peak memory consumption of a concrete input}
%	\label{fig:peak-input-memory-consumption}
%\end{figure}
%
%\begin{figure}[H]
%	\begin{tabular}{ l L L L}
%		Peak memory consumption & \pmemconsume{P}{\{ I_1,\cdots,I_n \}} & \bnfdef &
%		\max(\pmemconsume{P}{I_1},\cdots,\pmemconsume{P}{I_n})
%	\end{tabular}
%	\caption{Peak memory consumption of a set of inputs}
%	\label{fig:peak-inputs-memory-consumption}
%\end{figure}
%
%\begin{figure}[H]
%	\begin{tabular}{ l L L L}
%		Peak memory consumption & \pmemconsume{P}{S = \{ I \bnfalt I \vDash p \}} & \bnfdef &
%		\max_{I_i \in S}(\pmemconsume{P}{I_i})
%		\\
%		& & &
%		\hfill \text{where $P$ stands for a program, $S$ stands for a}
%		\\
%		& & &
%		\hfill \text{particular set of input, where every input}
%		\\
%		& & &
%		\hfill \text{satisfies constraint $p$}
%	\end{tabular}
%	\caption{Peak memory consumption of a particular set of inputs}
%	\label{fig:peak-memory-consumption}
%\end{figure}
\normalsize

\small
%\left.A\right.\vert_{B}
%\begin{figure}[H]
%	\begin{tabular}{ l L L L}
%		Peak memory consumption & \pmemconsume{P}{I} & \bnfdef &
%		\symmemconsume{\pathset}{I}{},
%		\text{where \pathset\;is a set of all possible call graph}
%		\\
%		& & &
%		\hfill \text{paths computed from $P$}
%		\\
%		Sym peak memory consumption & \symmemconsume{\pathset}{I}{} & \bnfdef &
%		\max_{\callpath_i \in \pathset}
%		(
%			\sum_{\env_{i_j} \in \callpath_i}^{}
%				(
%					\sum_{x \in \domof{\env_{i_j}}}^{} \symreachheap{x:\ty}{\env_{i_j}}
%				)
%			\biggl.\lvert_{I}
%		),
%		\\
%		& & &
%		\hfill \text{where\;} \pathset = \{\callpath_i \bnfalt \callpath_i=\env_{i_1}\env_{i_2}\cdots \}
%		\\
%		Sym peak reachable heap size & \symreachheap{x:\ty}{\env} & \bnfdef &
%		4
%		\text{,\;where\;} \ty=\kwint
%		\\
%		& & &
%		1
%		\text{,\;where\;} \ty=\kwbool
%		\\
%		& & &
%		\sizeof{x}
%		\text{,\;where\;} \ty=\kwlist, \sizeof{x} \text{\;is a symbolic expression}
%		\\
%		& & &
%		\hfill \text{that represents variable $x$'s max possible size}
%		\\
%		& & &
%		\hfill \text{in terms of other variables' symbolic size in } \env
%%		\\
%%		& & &
%%		\hfill \text{if reached from a valid call graph path}
%		\\
%		& & &
%		\sum_{f \in C}^{} \symreachheap{x.f:\ty_f}{\env}
%		\text{,\;where\;} \ty=C
%	\end{tabular}
%	\caption{Peak memory consumption}
%\label{fig:peak-memory-consumption}
%\end{figure}
\normalsize

\begin{figure}[H]
	\begin{tikzpicture}
	
	\tikzset{vertex/.style = {shape=rectangle,draw,minimum size=1.5em}}
	\tikzset{edge/.style = {->,> = latex'}}
	% vertices
	%	\node[vertex] (list) at  (3,7.5) {\kwlist};
	\node[vertex] (top) at  (3,4.5) {\trefine{\kwlist}{\kwtop}};
	%	\node[vertex] (bounded) at  (3,4.5) {\trefine{\kwlist}{\invbounded}};
	\node[vertex] (pred1) at  (0,3) {\trefine{\kwlist}{\inv{\kwpredicate_1}}};
	\node[vertex] (predn) at  (6,3) {\trefine{\kwlist}{\inv{\kwpredicate_n}}};
	\node[vertex] (bottom) at  (3,1.5) {\trefine{\kwlist}{\kwbottom}};
	%edges
	%	\draw[edge] (list) to (top);
	\draw[edge] (top) to (pred1);
	\draw[edge] (top) to (predn);
	%	\draw[edge] (bounded) to (pred1);
	%	\draw[edge] (bounded) to (predn);
	\draw[edge] (pred1) to (bottom);
	\draw[edge] (predn) to (bottom);
	%	\draw[edge] (a)  to[bend left] (a1);
	
	\path (pred1) to node {\dots} (predn);
	\node [shape=circle,minimum size=1.5em] (invisible1) at (2,3) {};
	\node [shape=circle,minimum size=1.5em] (invisible2) at (4,3) {};
	\end{tikzpicture}
	\caption{List type hierarchy}
	\label{fig:list-type-hierarchy}
\end{figure}



\subsection{Bounded lists}
\label{subsec:bounded-lists}

This section aims at proving \emph{every list} in the program will have a bounded length, as long as type checking succeeds by following rules in Figure \ref{fig:typingrules}.
Formally, \emph{every list} here refers to syntactic lists --- local list variables, class fields of list type, and local variables' fields if the field is of list type.
The overall strategy is to prove every type checking rule either satisfies \textbf{creation} or \textbf{preservation} --- if every newly \textbf{created} object has a bounded length and every other statement \textbf{preserves} the boundedness, then the proof is done.

\paragraph{Creation}
For every statement, it will be successfully type checked if and only if
\begin{itemize}
	\item A statement creates a new object, and any list that is directly or indirectly reachable from the object has a bounded length. (, )
\end{itemize}

In rule , $x$'s type has to make sure the new list's length is bounded.

In rule , the type rule enforces the restriction that if class $C$ has a field of list type, then there has to be a bound on the field of any instance of class $C$.
The boundedness either comes from class field declaration when there is no annotation on $x.f$, or comes from local variable declaration (when there is annotation on $x.f$).
%We have several cases to consider.
%If $x.f$ has default annotation, 
Note that \;only guarantees boundedness for $C$'s directly accessible field, instead of a field with a longer access path.
However, \;is sound because it also makes sure that object creation of a variable reachable from $C$'s field will have its field bounded.
For example, $h$ has a bounded length in $C.g.h$, if $C.g$.

\paragraph{Preservation}
For every statement, it will be successfully type checked if and only if
\begin{itemize}
	\item A statement is an assignment without creating new objects, and the boundedness of rhs is preserved in lhs. (, , )
	\item A statement is able to modify any invariant, and the invariant is preserved after executing itself. (, )
	\item A statement's subcomponents will type check. (, , )
	\item A statement has nothing to do with memory bounding. (, , , )
\end{itemize}

Rule \;is standard. It checks the subtyping relation between lhs $y$ and rhs $x$.
If $x$ and $y$ are both class type, then $x$'s reachable fields and $y$'s reachable fields?.
If $x$ and $y$ are both list type, then according to the type hierarchy in Figure \ref{fig:list-type-hierarchy}, $y$'s length will not go unbounded if $x$'s length is bounded.
Note that since $y$ cannot be type \trefine{\kwlist}{} (see Section \ref{subsec:type-system}), $y$'s type will always be subtype of \trefine{\kwlist}{?}.

Rule  not only checks subtyping relation between lhs $y$ and rhs $x.f$, but also checks the subtyping relation between the declared field type $\ty_f'$ and lhs $y$.
In other words,  $y$ is a super type of both $x.f$'s declared class field type and object field type.
The proof for rule \;is similar.

Rule ,  and \;are inductive cases.
Rule , ,  and \;has no influence on boundedness.

\subsection{Bounded program}
\label{subsec:bounded-program}

\paragraph{Lemma 2}

Also note that in Object-Oriented Programming, it looks unsound at the first glance to only consider local variables, because an object's actual memory consumption is not only , but also . . However, .
when an object has a field that is a collection data structure, transitive size.
list of object, each object has a list: rare case, require the invariant also consider increasing sizes of reachable objects

After successfully validating invariants, we will informally but soundly prove that this program will consume a bounded amount of memory under an input budget, by making sure the following assertions hold true
\begin{enumerate}
	\item Every local list variable created by new instruction, class field with a list type and/or all instances of a class that are created by new instruction and have a list field are annotated by an invariant in its type specification, where the invariant specifies the relation between length of the list and other variable(s).
	\item In every invariant, the value of rhs is bounded. Therefore the list variable represented by \code{<self> on lhs} has a bounded length.
	\item It over-approximates memory usage of the original program to assume that every local variable have exactly one copy in the memory at the same time.
	\item Every local variable has a bounded \emph{deep size}.
	\item Every list variable's length is bounded by some other list variables, except the input lists.
\end{enumerate}
The user is responsible for guaranteeing (1) and (4). But we argue the annotation burden for a user is not heavy, because he is free to leave lists unannotated, when he realizes a list variable will not contribute to memory consumption (e.g. the alias of a list). The implicit annotation for any unannotated list is \code{Top}, meaning that the list does not contribute to memory consumption.
Regarding (4), deep size. %TODO: whether it is appropriate to mention it here?


(3) is a valid assertion for a Java web application when there is no recursive methods and no recursive types.
We argue that \circled{1} recursive methods should not influence the memory boundedness of a program, and \circled{2} assuming no recursive types is reasonable when reasoning about memory boundedness of a web application.
First of all, the intuition of (3) comes from the point of view of garbage collection. After returning to the caller, a method's local variables will be garbage collected if they do not escape the local scope.
There are two ways to escape --- either stored into a class field or a collection data structure. While the former case does not invalidate (3) because of being explicitly considered, the latter case is also soundly captured by user-provided invariants.
However, there is actually a situation where (3)'s soundness is broken --- every local variable in a recursive method will possibly have more than one copy in the stack.
Nevertheless, in reality the stack space of a program is usually bounded and is smaller in orders of magnitude than heap space. Therefore, from the perspective of concerning memory consumption, it is reasonable not to consider stack space.
One exception here would be that there are list variables in recursive methods, under which scenario the boundedness of stack space won't guarantee the boundedness of heap space. However, in reality we have not yet found such a case.
Recursive types will also make (3) an unsound over-approximation, because they will lead to the situation where a local variable points to an unbounded amount of heap cells (e.g. node in a linked list).
However, recursive types are usually used to implement collection data structures whose sizes could grow arbitrarily large. In real life programs (including web applications), we discovered that it is a rare case that a programmer implements his own collection data structures. Instead, he will be very likely to use library APIs, which is exactly modeled by list-abstraction.

\begin{figure}
	\begin{lstlisting}[language=java]
	List<String> input;
	@Inv("self+rem(input)=c9-c8+input_init") List<Object> blogDB;
	@Inv("input") Iterator<Object> it;
	it = input.iterator();
	while(true) {
	if (it.hasNext() && ndet()) {
	String blog;
	c8: blog = it.next();
	c9: blogDB.add(blog);
	} else if (it.hasNext() && ndet()) {
	String keyword;
	keyword = it.next();
	@Inv("self+rem(blogDB)=c25-c18-c26+len(blogDB)") List<String> toShow;
	@Iter("blogDB") Iterator it2;
	it2 = blogDB.iterator();
	String b;
	if (it.hasNext()) {
	c18: b = it.next();
	b = "Blog begins:\n" + b;
	while(true) {
	if (it.hasNext()) {
	if (...) // Determine if the blog contains any sensitive word
	return;
	if (b.contains(keyword))
	c25: toShow.add(b);
	c26: b = it.next();
	}
	}
	} // render toShow on an HTML page
	} }
	\end{lstlisting}
	\caption{Motivating example}
	\label{fig:motivating-example}
\end{figure}

%Different callback orderings cause different memory usage of list \code{toShow}.
%For example, list \code{toShow}'s length is either 1 or 0 if we alternate the order of executing \code{postNewBlog} once and executing \code{showBlogs} once.













%on evaluation rules in Figure \ref{fig:operational-semantic}. The proof is done by induction on every evaluation rule in Figure \ref{fig:operational-semantic}.

%\paragraph{Lemma 1}
%If $\subtyof{\ty_1}{\ty_2}$, then 
%$\evalty{x_1}{\tyenv_1,x_1:\ty_1}{\env_1}
%\implies
%\evalty{x_2}{\tyenv_2,x_2:\ty_2}{\env_2}$, where typing contexts $\tyenv_1$ and $\tyenv_2$ are free variables, environments $\env_1$ and $\env_2$ are also free variables.
%
%\paragraph{Proof}
%We prove Lemma 1 by induction on type $\ty_1$'s and type $\ty_2$'s structures.
%The base cases are when type $\ty_1$ and type $\ty_2$ are both $\kwint$, $\kwbool$ or $\kwiterator$.
%Here Lemma 1 obviously holds true according to Rule \textsc{<:Int}, \textsc{<:Bool}, \textsc{<:Iter} and \textsc{V-Base}.
%
%In the inductive case, we will split on cases where type $\ty_1$ and type $\ty_2$ are both in a structure like $\tlist{\ty}$ or $\trefine{\ty}{\kwrefine}$.
%\begin{itemize}
%	\item If type $\ty_1$ and type $\ty_2$ are both in a structure like $\tlist{\ty}$, then due to Rule \textsc{<:List}, we have $\subtyof{\ty_{1_e}}{\ty_{2_e}}$, where variable $x_{1_e}$ and variable $x_{2_e}$ represent an element of list $x_1$ and list $x_2$, respectively.
%	
%	According to inductive assumption, we have
%	$\evalty{x_{1_e}}{\tyenv_1,x_1:\ty_{1_e}}{\env_2}
%	\implies
%	\evalty{x_{2_e}}{\tyenv_2,x_2:\ty_{2_e}}{\env_2}$ holds true.
%	
%	Then according to Rule \textsc{V-BaseList}, our goal is to prove: if $a_1 \implies b_1 \cdots a_n \implies b_n$ then $(a_1 \land\cdots\land a_n)\implies(b_1 \land\cdots\land b_n)$, where each term $a_i$ is $\evalty{x_{1_e}}{\tyenv,x_1:\ty_{1_e}}{\mapext{\env}{x_{1_e}}{v_{1_e}}}$ and each term $b_i$ is $\evalty{x_{2_e}}{\tyenv,x_2:\ty_{2_e}}{\mapext{\env}{x_{2_e}}{v_{2_e}}}$.
%	
%	To prove our goal, we first transform $(a_1 \land\cdots\land a_n)\implies(b_1\land\cdots\land b_n)$ into $\neg(a_1 \land\cdots\land a_n) \lor (b_1 \land\cdots\land b_n)$.
%	Then we consider two cases:
%	\begin{itemize}
%		\item Every term $a_i$ is $\kwtrue$. Then every term $b_i$ has also to be $\kwtrue$. Therefore we have proven its validity because $(b_1 \land\cdots\land b_n)$ is $\kwtrue$.
%		\item There is at least one term $a_i$ that is $\kwfalse$. Then we have also proven its validity because $\neg(a_1 \land\cdots\land a_n)$ is $\kwtrue$.
%	\end{itemize}
%
%	\item If type $\ty_1$ and type $\ty_2$ are both in a structure like $\trefine{\ty}{\kwrefine}$ (let $\ty_1$ be $\trefine{\ty_{1_B}}{\kwrefine_1}$ and $\ty_2$ be $\trefine{\ty_{2_B}}{\kwrefine_2}$), then according to Rule \textsc{<:Refine}, we have $\subtyof{\ty_{1_B}}{\ty_{2_B}}$ and $\kwrefine_1\implies\kwrefine_2$ holds true.
%	
%	According to Rule \textsc{V-Refine}, our goal is to prove: if $a_1 \land b_1$ then $a_2 \land b_2$, where term $a_1$ is $\evalszexpr{\kwrefine_1}{x_1}{\env}$, term $b_1$ is $\evalty{x_1'}{\tyenv_1,x_1':\ty_{1_B}}{\env_1}$, term $a_2$ is $\evalszexpr{\kwrefine_2}{x_2}{\env}$, and term $b_2$ is $\evalty{x_2'}{\tyenv_2,x_2':\ty_{2_B}}{\env_2}$.
%	
%	Since we have (1) $\kwrefine_1\implies\kwrefine_2$ holds for \textbf{arbitrary} free variables in $\kwrefine_1$ (or $\kwrefine_2$) and (2) $\evalszexpr{\kwrefine_1}{x_1}{\env}$ (or $\evalszexpr{\kwrefine_2}{x_2}{\env}$) is one possible binding of free variables for $\kwrefine_1$ (or $\kwrefine_2$) according to Figure \ref{fig:type-semantic}, \ref{fig:refinement-init-val} and \ref{fig:gen-constraint}, we have $a_1 \implies a_2$.
%	According to inductive assumption and $\subtyof{\ty_{1_B}}{\ty_{2_B}}$, we have $b_1 \implies b_2$.
%	Then we goal is proven.
%\end{itemize}
%Intuitively, Lemma 1 says that subtyping relation between two variables guarantees the implication relation between their size constraints, regardless of the typing context or environment.
%
%
%\begin{itemize}
%	\item Rule \textsc{E-IfExpr, E-IfTrue, E-IfFalse, E-While}: Updated environment $\env'$ is obviously well-sized because there is no update in the environment.
%	
%	\item Rule \textsc{E-BlockqSkip}: Updated environment $\env'$ is obviously well-sized because there is no update in the environment.
%	Next statement $\stmt'$ will type check because of the premises in Rule \textsc{T-Block}.
%	
%	\item Rule \textsc{E-Block}: Updated environment $\env'$ is well-sized if the updated environment $\env'$ is well sized for all other evaluation rules (which is being proven).
%	
%	\item Rule \textsc{E-Label}: Updated environment $\env'$ will type check because (1) the transition in Rule \textsc{E-Label} is an intermediate state transition and updated environment $\env'$ is the consequence of applying evaluation rules for basic statements, (2) type check happens in premise of Rule \textsc{T-Label}, where the label is incremented by 1 for all type checking rules for basic statements (Rule \textsc{T-Add, T-Remove, T-Next, T-Assign, T-Skip, T-Decl}).
%	Note that when a line counter is used to label more than one basic statement, type checking statement $\stmt$ makes sure that a counter increment in Rule \textsc{E-Label} is always checked in one of the type checking rules for basic statements.
%	
%	\item Rule \textsc{E-Var, E-ArithL, E-ArithR, E-CompL, E-ComR, E-LogicL, E-LogicR, E-Neg, E-Iterator, E-HasNext, E-AssignExpr}: Updated environment $\env'$ is obviously well-sized because there is no update in the environment.
%	Note that Rule \textsc{T-Var, T-Arith, T-Comp, T-Logic, T-Neg, T-Iterator, T-HasNext} \textbf{infer} the type of an expression.
%	Rule \textsc{T-Var} collects a conjunction of constraints together with variable $x$'s declared type as the actual type of variable $x$, where each clause in the conjunction is a constraint generated from a type that is dependent on variable $x$.
%	
%	\item Rule \textsc{E-Assign}: Rule \textsc{T-Assign} checks	if predicates on expression $e$ entails predicates on variable $x$. If succeeds, predicates on variable $x$ will still hold after assignment, since predicates on expression $e$ holds before assignment according to inductive assumption.
%	Note that predicates on $e/x$ is the conjunction of all types that are dependent on $e/x$ together with $e/x$'s declared type, due to Rule \textsc{T-Var}.
%	
%	Rule \textsc{T-Assign} indicates that \textbf{principle of substitution} is admissible in our type system: In any type refinement that uses expression $e$, variable $x$ could be substituted for expression $e$ in the refinement.
%	Therefore, type of every variable is still satisfiable after Rule \textsc{E-Assign}, i.e. the environment after an evaluation step is well-sized.
%	
%	\item Rule \textsc{E-Next}: In the environment, each line counter $\counter$ in the counter environment $\counterenv$ is incremented by 1, remainder of $x$ is decremented by 1 and $y$ is assigned the value of an element from list $z$.
%	Therefore, due to the fact that flow-insensitiveness over-approximates execution traces of the original program, Rule \textsc{T-Next} checks for each type in the type environment, if these updates will lead to unsatisfiability.
%\end{itemize}
%
%We prove refinement preservation by induction on each evaluation step.
%Assume refinement preservation holds true for evaluation step $k$, then we will split cases on each possible evaluation rule that could be applied at step $k+1$ in order to prove $\tycheck{\tyenv}{\env'}\land\tycheck{\tyenv}{\stmt'}$ holds true.
%
%Rule \textsc{E-Add}: Statement $\stmt'$ is $\eskip$, which type checks according to Rule \textsc{T-Skip}.
%
%Next we prove $\evalty{x}{\tyenv}{\env}$ holds true for every $(w:\ty_w)\in\tyenv'$.
%
%\begin{itemize}
%	\item If variable $w$ has no explicit refinement, then we delegate this to the case of explicit refinements, by soundly augmenting variable $w$ with an explicit refinement $\kwtrue$.
%	
%	\item If variable $w$ has an explicit refinement (let $\ty_w$ be $\trefine{\ty_W}{\kwrefine_W}$), then we need to prove $\evalty{w}{\tyenv}{\env'}$ holds true.
%	According to Rule \textsc{V-Refine}, we then decompose the goal into proving the validity of $\evalszexpr{\kwrefine_W}{w}{\env'}$ and $\evalty{w'}{\tyenv,w':\ty_w}{\mapext{\env'}{w'}{\env'[w]}}$, where variable $w'$ is a fresh variable that has the same value and type as variable $w$.
%	
%	When evaluating the value of $\evalszexpr{\kwrefine_W}{w}{\env'}$, we see that Rule \textsc{T-Add} makes sure that the updated value of refinement $\kwrefine_W$ in environment $\env'$ is entailed by its original value in environment $\env$.
%	Since the original value in environment $\env$ is evaluated to $\kwtrue$ according to inductive assumption, its new value will also holds true in environment $\env'$.
%	\begin{itemize}
%		\item For every iterator $z$ that is attached to list $y$, value of $\evalszexpr{\rem{z}}{w}{\env'}$ is incremented by 1 compared with its value in environment $\env$, according to Rule \textsc{E-Add} and \textsc{V-Rem}.
%		\item Value of $\evalszexpr{\len{y}}{w}{\env'}$ is incremented by 1 compared with its value in environment $\env$, according to Rule \textsc{E-Add} and \textsc{V-Len}.
%		\item Value of $\evalszexpr{\counter}{w}{\env'}$ is incremented by 1 compared with its value in environment $\env$,  according to Rule \textsc{E-Add} and \textsc{V-Counter}.
%		\item Value of $\evalszexpr{\kwself}{w}{\env'}$ is incremented by 1 compared with its value in environment $\env$ if $w \equiv y$, according to Rule \textsc{E-Add} and \textsc{V-List}.
%	\end{itemize}
%	
%	When evaluating the value of $\evalty{w'}{\tyenv,w':\ty_w}{\mapext{\env'}{w'}{\env'[w]}}$, we only need to consider when $\env'[w] \equiv \env'[y]$, because all other values in the environment are unmodified according to Rule \textsc{E-Add}.
%	Next we split on two cases: variable $w'$ is or is not a list.
%	
%	\begin{itemize}
%		\item Variable $w'$ cannot not be a list, because the base type checking would eliminate this situation.
%%		$\evalty{w'}{\tyenv,w':\ty_w}{\mapext{\env'}{w'}{\env'[w]}}$ holds true according to Rule \textsc{V-Base}.
%		
%		\item When variable $w'$ is a list, we only need to prove $\evalty{x'}{\tyenv,x':\ty_{y_e}}{\mapext{\env'}{x'}{\env'[x]}}$ according to Rule \textsc{V-BaseList} (where variable $x'$ is a fresh variable that has a same value as the last element in list $y$ and has the same type as list $y$'s elements), because the rest elements in list $y$ do not change their values according to Rule \textsc{E-Add}.
%		
%		According to Lemma 1 and the subtype check in Rule \textsc{T-Add} between type $\ty_x$ and type $\ty_{y_e}$, we have
%		$\evalty{x}{\tyenv}{\env}
%		\implies \evalty{x'}{\tyenv,x':\ty_{y_e}}{\mapext{\env'}{x'}{\env'[x]}}$.
%		
%		According to inductive assumption, we have $\evalty{x}{\tyenv}{\env}$.
%		Therefore, we have proven our goal.
%%		Note that variable $w'$'s value is the same as variable $x$'s since variable $x$'s value is appended into list $y$.
%	\end{itemize}
%\end{itemize}
%
%Rule \textsc{E-Remove}: The proof is similar to Rule \textsc{E-Add}.
%
%Rule \textsc{E-Assign}: Statement $\stmt'$ is $\eskip$, which type checks according to Rule \textsc{T-Skip}.
%
%Next we prove that $\evalty{v: \ty}{\env}$ holds true for every $(w:\ty_w)\in\tyenv'$.
%
%\begin{itemize}
%	\item If variable $w$ has no explicit refinement, then we delegate this to the case of explicit refinements, by soundly augmenting variable $w$ with an explicit refinement $\kwtrue$.
%	
%	\item If variable $w$ has an explicit refinement (let $\ty_w$ be $\trefine{\ty_W}{\kwrefine_W}$), then we need to prove $\evalty{w}{\tyenv}{\env'}$ holds true.
%	According to Rule \textsc{V-Refine}, we then decompose the goal into proving the validity of $\evalszexpr{\kwrefine_W}{w}{\env'}$ and $\evalty{w'}{\tyenv,w':\ty_w}{\mapext{\env'}{w'}{\env'[w]}}$, where variable $w'$ is a fresh variable that has the same value and type as variable $w$.
%	
%	When evaluating the value of $\evalszexpr{\kwrefine_W}{w}{\env'}$
%\end{itemize}

==> types-and-refinements.tex <==




